Quark mass effects in two-loop Higgs amplitudes

We provide two two-loop amplitudes relevant for precision Higgs physics. The first is the two-loop amplitude for Higgs boson production through gluon fusion with exact dependence on the top quark mass up to squared order in the dimensional regulator $\epsilon$. The second result we provide is the two-loop amplitude for the decay of a Higgs boson into a pair of massive bottom quarks through the Higgs-to-gluon coupling in the infinite top mass limit. Both amplitudes are computed by finding canonical bases of master integrals, which we evaluate explicitly in terms of harmonic polylogarithms. We obtain the bare, renormalized and IR-subtracted amplitude and provide the results in terms of building blocks suitable to changing renormalization schemes.

==> amplitude_computation/mass_ct.tex <==
% !TEX root = main.tex
\begin{figure}[h!]
	\begin{center}
% y_t LO
		\begin{subfigure}{0.3\textwidth}
			\centering
     		\scalebox{1.5}{\begin{tikzpicture}[scale=0.9, every node/.style={scale=0.9}]
     		\begin{feynman}
     		\vertex (a);
			\vertex[below=1.5cm of a] (a2) ;
     		\vertex[right=0.5cm of a] (b) ;
			\vertex[right=0.5cm of a2] (b2);
     		\vertex[right=1.3cm of b] (c1);
			\vertex[below=0.75cm of c1] (c) [red,crossed dot] {};
     		\vertex [right=0.6cm of c] (d);
     		\diagram*{
     			(a) --[fermion, very thick] (b) --[fermion, very thick,insertion={[style=red,size=3pt]0.6}] (b2) --[fermion, very thick] (a2),
     			(c) -- [scalar] (d),
     			(c) --[gluon] (b) ,
				(c) -- [gluon] (b2),
     		};
			\vertex [above =1.1em of c] {$\textcolor{red}{C_1}$};
     		\end{feynman}
     		\end{tikzpicture}}
		\end{subfigure}
		\caption{Feynman diagram defining $\tilde{M}_{y_t,1}^0$. The dressed fermion propagator reads $G^{uv,\delta m}_{f,ij}(k)=\frac{i \delta_{ik}}{\slashed{k}-m_b^0}\left(-i m_b^0\right)\frac{i \delta_{k j}}{\slashed{k}-m_b^0}$ \label{fig:mass_ct_qqbH}}
	\end{center}	
\end{figure}

==> appendices/results_qqbH.tex <==
\begin{align}
-&\frac{i}{m_b^3} M_{y_t,2}^{fin}=
	\frac{16 \left(1+x^4\right) H_{-4}(x)}{3 x \left(-1+x^2\right)}
	-\frac{26 (1+x)^2 \log\left(\frac{\mu ^2}{m_b^2}\right){}^2}{x}
	\nonumber \\
	&
	-\frac{2 \pi ^2 (1049+x (-708+x (-2764+x (684+1355 x))))}{81 x \left(-1+x^2\right)}
	-\frac{32 \left(1+x^2\right) H_2(x){}^2}{9 x}
	\nonumber \\
	&
	-\frac{4 (17+x (-23+13 x (13+5 x))) H_3(x)}{9 x (1+x)}
	+\frac{4}{9} \left(92+\frac{107}{x}+59 x+\frac{144}{1+x}\right) \zeta_{3}
	\nonumber \\
	&
	-\frac{4 \pi ^2 (5+x (8+5 x)) \log(1+x)}{9 x}
	+\frac{(5+x (-54+x (-192+x (-54+125 x)))) \log(x)^4}{54 x \left(-1+x^2\right)}
	\nonumber \\
	&
	+\frac{64 (-1+x) (1+x (5+x)) H_{2,1}(x)}{3 x (1+x)}
	-\frac{8 (5+x (8+5 x)) H_{-3}(x)}{9 x}
	\nonumber \\
	&
	+\frac{(8+8 x (-18+x (-24+(-18+x) x))) H_4(x)}{3 x \left(-1+x^2\right)}
	-\frac{8993 (1+x)^2}{54 x}
	\nonumber \\
	&
	+H_{-2}(x) \left(-\frac{128 (1+x) \left(1+x^2\right)}{9 (-1+x) x}-\frac{\pi ^2 \left(88-40 x^4\right)}{27 x-27 x^3}-\frac{64 \left(1+x^2\right) H_2(x)}{9 x}\right)
	\nonumber \\
	&
	+\left(-\frac{4 (-1+x) (625+x (1292+625 x))}{27 x (1+x)}+\frac{16 \pi ^2 (4+x (27+x (25+(27-2 x) x)))}{27 x \left(-1+x^2\right)}\right) H_2(x)
	\nonumber \\
	&
	+\pi ^4 \left(-\frac{32}{15}-\frac{49}{15 (-1+x)}-\frac{277}{405 x}+\frac{31 x}{15}+\frac{1}{1+x}\right)
	\nonumber \\
	&
	+\log(1-x) \left(-\frac{4 (41+x (110+41 x))}{9 x}+\frac{\pi ^2 (-52+4 x (-1+x (91+31 x)))}{9 x (1+x)}
	\right.
	\nonumber \\
	&
	\left.
	-\frac{16 \pi ^2 \left(-1+x^2\right) \log(x)}{3 x}+\left(\frac{248}{9}+\frac{2}{x}+\frac{50 x}{3}-\frac{16}{1+x}\right) \log(x)^2-\frac{16 \left(-1+x^2\right) \log(x)^3}{3 x}
	\right.
	\nonumber \\
	&
	\left.
	+\left(32-\frac{88}{3 x}+\frac{88 x}{3}-\frac{64}{1+x}\right) H_2(x)\right)
	+\log\left(1+x^2\right)^2 \left(\frac{32 (1+x)^2}{9 x}+\frac{16 \pi ^2 \left(-1+x^2\right)}{27 x}
	\right.
	\nonumber \\
	&
	\left.
	+\frac{16 \left(-1+x^2\right) H_2(x)}{9 x}\right)
	+\log\left(\frac{\mu ^2}{m_b^2}\right) \left(-\frac{350 (1+x)^2}{3 x}
	\right.
	\nonumber \\
	&
	\left.
	-\frac{8 \pi ^2 (31+x (24+x (-116+x (12+25 x))))}{27 x \left(-1+x^2\right)}-\frac{16 (1+x (10+x)) \log(1-x)}{3 x}
	\right.
	\nonumber \\
	&
	\left.
	+\frac{(62+2 x (24+x (-134+x (-24+7 x)))) \log(x)^2}{9 x-9 x^3}+\frac{8 (1+x)^2 \log\left(1+x^2\right)^2}{3 x}
	\right.
	\nonumber \\
	&
	\left.
	+\log(x) \left(\frac{8}{3} \left(18+\frac{16}{-1+x}+\frac{1}{x}+x\right)+\frac{32 (1+x) \left(1+x^2\right) \log(1+x)}{3 (-1+x) x}-\frac{32 x (1+x) \log\left(1+x^2\right)}{3 (-1+x)}\right)
	\right.
	\nonumber \\
	&
	\left.
	-\frac{32 (1+x) \left(1+x^2\right) H_{-2}(x)}{3 (-1+x) x}-\frac{8 (-1+x) (31+x (86+31 x)) H_2(x)}{9 x (1+x)}\right)
	\nonumber \\
	&
	+\log(x)^2 \left(\frac{2}{27} \pi ^2 \left(\frac{1}{x}+51 x-\frac{6 (9+x (10+9 x))}{-1+x^2}\right)
	\right.
	\nonumber \\
	&
	\left.
	+\frac{533+x (-659+x (-1864+3 x (296+(233-175 x) x)))}{27 (-1+x)^2 x (1+x)}-\frac{4 (5+x (8+5 x)) \log(1+x)}{9 x}
	\right.
	\nonumber \\
	&
	\left.
	+\frac{4 \left(-1+x^2\right) \log\left(1+x^2\right)^2}{9 x}-\frac{8 \left(-3+x^4\right) H_{-2}(x)}{9 x \left(-1+x^2\right)}+\frac{16 \left(4-7 x^2+4 x^4\right) H_2(x)}{9 x-9 x^3}\right)
	\nonumber \\
	&
	+\log(x)^3 \left(-\frac{2 (34+x (82+x (-139+x (2+65 x))))}{27 x \left(-1+x^2\right)}+\frac{16 \left(1+x^2\right) \log(1+x)}{9 x}
	\right.
	\nonumber \\
	&
	\left.
	-\frac{16}{9} x \log\left(1+x^2\right)\right)+\log(x) \left(\frac{4 (69+x (138+41 x))}{9 (-1+x)}
	\right.
	\nonumber \\
	&
	\left.
	-\frac{8 \pi ^2 (11+(-1+x) x (-29+x (-1+16 x)))}{27 x \left(-1+x^2\right)}+\frac{8 \left(1+x^4\right) \zeta_{3}}{9 x-9 x^3}
	\right.
	\nonumber \\
	&
	\left.
	+\frac{32 \left(1+x^4\right) H_{-3}(x)}{9 x-9 x^3}
	\right.
	\nonumber \\
	&
	\left.
	+\frac{8 (5+x (8+5 x)) H_{-2}(x)}{9 x}+\frac{4}{3} \left(52+\frac{17}{x}+11 x-\frac{24}{1+x}\right) H_2(x)
	\right.
	\nonumber \\
	&
	\left.
	+\log\left(1+x^2\right) \left(-\frac{64 \pi ^2 x}{27}-\frac{128 x (1+x)}{9 (-1+x)}-\frac{64}{9} x H_2(x)\right)
	\right.
	\nonumber \\
	&
	\left.
	+\log(1+x) \left(\frac{64 \pi ^2 \left(1+x^2\right)}{27 x}+\frac{128 (1+x) \left(1+x^2\right)}{9 (-1+x) x}+\frac{64 \left(1+x^2\right) H_2(x)}{9 x}\right)
	\right.
	\nonumber \\
	&
	\left.
	+\frac{32 \left(1+x^4\right) H_3(x)}{9 x \left(-1+x^2\right)}\right)
\end{align}

==> computation_mis/mis_LO_explicit.tex <==
\begin{align}
	f_1^I
		=& \sum_{n=0}^{\infty} \epsilon^i {f}_{1,n}^{I}
		= \epsilon  I_{0,0,2}
		=e^{\gamma_E  \epsilon } \epsilon  \Gamma (\epsilon )
		\nonumber 
		\\
		=&
		1
		+\epsilon^2 \frac{\pi ^2}{12}
		-\epsilon^3\frac{\zeta_{3}}{3}
		+\epsilon^4\frac{\pi ^4}{160}
		+\mathcal{O}\left(\epsilon^5\right)
	\\
	%
	f_2^I
		=& \sum_{n=1}^{\infty} \epsilon^i {f}_{2,n}^{I}
		= \epsilon \frac{\left(x^2-1\right)   m_t^2}{x}I_{0,1,2} 
		\nonumber
		\\
		=&
		-\epsilon \log (x)
		+\frac{\epsilon^2}{6} \left[-12 H_{-2}(x)-3 \log ^2(x)+12 \log (x+1) \log (x)+\pi ^2\right]
		\nonumber
		\\
		&+\epsilon^3\bigg[
			-4 H_{-2,-1}(x)-2 H_{-3}(x)+\log (x+1) \left(4 H_{-2}(x)+\log ^2(x)-\frac{\pi ^2}{3}\right)
			\nonumber
			\\
			&\ \ \qquad
			-\frac{1}{6} \log ^3(x)-2 \log ^2(x+1) \log (x)+\frac{1}{12} \pi ^2 \log (x)+2 \zeta_{3}
		\bigg]
		\nonumber
		\\
		&+\epsilon^4
		\bigg[
			-4 H_{-3,-1}(x)-8 H_{-2,-1,-1}(x)+8 \log (x+1) H_{-2,-1}(x)-2 H_{-4}(x)
			\nonumber
			\\
			& \ \ \qquad 
			-\frac{1}{6} H_{-2}(x) \left(24 \log ^2(x+1)+\pi ^2\right)+4 H_{-3}(x) \log (x+1)+\frac{7}{3} \zeta_{3} \log (x)
			\nonumber
			\\
			& \ \ \qquad 
			-4 \zeta_{3} \log(x+1)-\frac{1}{24} \log ^4(x)+\frac{1}{3} \log (x+1) \log ^3(x)
			\nonumber
			\\
			& \ \ \qquad 
			+\frac{4}{3} \log ^3(x+1) \log (x)-\log ^2(x+1) \log ^2(x)+\frac{1}{24} \pi ^2 \log ^2(x)
			\nonumber
			\\
			& \ \ \qquad 
			+\frac{1}{3} \pi ^2 \log^2(x+1)-\frac{1}{6} \pi ^2 \log(x+1) \log (x)+\frac{7 \pi ^4}{180}
		\bigg]
		+ \mathcal{O}\left(\epsilon^5\right)
	\\
	%
	f_3^I
		=& \sum_{n=2}^{\infty} \epsilon^i {f}_{3,n}^{I}
		= -\epsilon ^2\frac{(x-1)^2   m_t^2}{x}I_{1,1,1}
		\nonumber
		\\
		=&
		\epsilon^2 \frac{\log ^2(x)}{2}
		+\epsilon^3
		\bigg[
			4 H_{-3}(x)-2 H_{-2}(x) \log (x)+\frac{\log ^3(x)}{6}-\frac{1}{6} \pi ^2 \log (x)-3 \zeta_{3}
		\bigg] 
		\nonumber
		\\
		&+\epsilon^4
		\bigg[
			4 \log (x) H_{-2,-1}(x)-2 H_{-2}(x){}^2+\frac{1}{3} H_{-2}(x) \left(\pi ^2-3 \log ^2(x)\right)
			\nonumber
			\\
			& \ \ \qquad 
			+2 H_{-3}(x) \log (x)-2 \zeta_{3} \log (x)+\frac{\log ^4(x)}{24}-\frac{1}{24} \pi ^2 \log ^2(x)-\frac{\pi ^4}{72}
		\bigg]
		\nonumber
		\\
		&+ \epsilon^5
		\bigg[
			24 H_{-4,-1}(x)+8 H_{-3,-2}(x)+8 H_{-2}(x) H_{-2,-1}(x)-\frac{2}{3} \pi ^2 H_{-2,-1}(x)
			\nonumber
			\\
			& \ \ \qquad 
			-32 H_{-3,-1,-1}(x)-16 H_{-2,-2,-1}(x)+2 \log ^2(x) H_{-2,-1}(x)-4 \log (x) H_{-3,-1}(x)
			\nonumber
			\\
			& \ \ \qquad 			
			-8 \log (x) H_{-2,-1,-1}(x)+4 \zeta(3) H_{-2}(x)+4 H_{-5}(x)-\frac{1}{3} H_{-2}(x) \log ^3(x)
			\nonumber
			\\
			& \ \ \qquad 
			+H_{-3}(x) \left(\log ^2(x)-4 H_{-2}(x)\right)-2 H_{-4}(x) \log (x)+\frac{1}{6} \pi ^2 H_{-2}(x) \log (x)
			\nonumber
			\\
			& \ \ \qquad 			
			-\frac{7}{6} \zeta_{3} \log ^2(x)+\frac{\log^5(x)}{120}-\frac{1}{72} \pi ^2 \log ^3(x)-\frac{7}{180} \pi ^4 \log (x)-7 \zeta_{5}+\frac{\pi ^2 \zeta_{3}}{12}
		\bigg]
		\nonumber
		\\
		&+ \epsilon^6
		\bigg[
			-8 \zeta_{3} H_{-2,-1}(x)+\frac{1}{6} H_{-3}(x) \left(48 H_{-2,-1}(x)+2 \log ^3(x)-\pi ^2 \log (x)-32 \zeta_{3}\right)
			\nonumber
			\\
			& \ \ \qquad 
			+8 H_{-2,-1}(x){}^2-8 H_{-2}(x) H_{-3,-1}(x)+\frac{2}{3} \pi ^2 H_{-3,-1}(x)-16 H_{-2}(x)
		    H_{-2,-1,-1}(x)
			\nonumber
			\\
			& \ \ \qquad 
			+\frac{4}{3} \pi ^2 H_{-2,-1,-1}(x)+\frac{2}{3} \log ^3(x) H_{-2,-1}(x)-2 \log ^2(x) H_{-3,-1}(x)
			\nonumber
			\\
			& \ \ \qquad 
			-4 \log ^2(x) H_{-2,-1,-1}(x)+4 \log (x) H_{-4,-1}(x)-\frac{1}{3} \pi ^2 \log (x) H_{-2,-1}(x)
			\nonumber
			\\
			& \ \ \qquad 
			+8 \log (x) H_{-3,-1,-1}(x)+16 \log (x) H_{-2,-1,-1,-1}(x)+\frac{14}{3} \zeta_{3} H_{-2}(x) \log (x)
			\nonumber
			\\
			& \ \ \qquad 
			+2 H_{-3}(x){}^2-\frac{1}{6} \pi ^2 H_{-2}(x){}^2+\frac{7}{90} \pi ^4 H_{-2}(x)-\frac{1}{12} H_{-2}(x) \log^4(x)
			\nonumber
			\\
			& \ \ \qquad 
			+\frac{1}{12} \pi ^2 H_{-2}(x) \log ^2(x)+\frac{1}{3} H_{-4}(x) \left(-12 H_{-2}(x)-3 \log ^2(x)+\pi ^2\right)
			\nonumber
			\\
			& \ \ \qquad 
			+2 H_{-5}(x) \log (x)-\frac{7}{18} \zeta_{3} \log ^3(x)-6 \zeta_{5} \log (x)+\frac{2}{9} \pi^2 \zeta_{3} \log (x)
			\nonumber
			\\
			& \ \ \qquad 
			+\frac{\log ^6(x)}{720}-\frac{1}{288} \pi ^2 \log^4(x)-\frac{47 \pi ^4 \log ^2(x)}{2880}+3 \zeta_{3}^2-\frac{23 \pi ^6}{4320}
		\bigg]
		+\mathcal{O}\left(\epsilon^7\right)
		\ ,
\end{align}
